SCL: A Secure Concurrency Layer For Paranoid Stateful Lambdas

We propose a federated Function-as-a-Service (FaaS) execution model that provides secure and stateful execution in both Cloud and Edge environments. The FaaS workers, called Paranoid Stateful Lambdas (PSLs), collaborate with one another to perform large parallel computations. We exploit cryptographically hardened and mobile bundles of data, called DataCapsules, to provide persistent state for our PSLs, whose execution is protected using hardware-secured TEEs. To make PSLs easy to program and performant, we build the familiar Key-Value Store interface on top of DataCapsules in a way that allows amortization of cryptographic operations. We demonstrate PSLs functioning in an edge environment running on a group of Intel NUCs with SGXv2. As described, our Secure Concurrency Layer (SCL), provides eventually-consistent semantics over written values using untrusted and unordered multicast. All SCL communication is encrypted, unforgeable, and private. For durability, updates are recorded in replicated DataCapsules, which are append-only cryptographically-hardened blockchain with confidentiality, integrity, and provenance guarantees. Values for inactive keys are stored in a log-structured merge-tree (LSM) in the same DataCapsule. SCL features a variety of communication optimizations, such as an efficient message passing framework that reduces the latency up to 44x from the Intel SGX SDK, and an actor-based cryptographic processing architecture that batches cryptographic operations and increases throughput by 81x.

==> design_old.tex <==
% ecalls/ocalls overhead 
\section{\algname Design}
\label{sec:scl}

\subsection{Overall Architecture}
% \todo{Eric}
\todo{a graph similar to the one on the slides, with components}
\todo{talk about that graph and overview the techniques} 
% \todo{}
% \todo{what we have: }
% \todo{DC: DataCapsule data structure, DataCapsule server(third party audit)}
% \todo{KVS: KVS, consistency, (Will's checkpoint?)}
% \todo{enclave: circular buffer, attestation} 
% \todo{optimization: multi threading}


The essence of \algname is that every secure enclave replicates a secure, append-only, and durable blockchain called a DataCapsule (Section \ref{sec:dc}). If two enclaves have the same replica of the hash chain, they yield the same KVS in memory. As a result, the goal of \algname is to efficiently propagate changes and consistently maintain the structure of a DataCapsule. 

Figure \ref{fig:overview} provides an overview of \algname's architecture. All the KVS updates by \texttt{put} are converted into a record appended to the DataCapsule hash chain. The DataCaspule record appends are propagated by a network multicast tree (Section \ref{sec:mcast}). If an enclave receives a record to append, it verifies the cryptographic signatures and hashes, and merges the record with its own replica of the DataCapsule. The merge does not require explicit coordination due to the CRDT property of the DataCapsule hash chain, but the hash chain is periodically synchronized to bound the consistency. The DataCapsule changes are also reflected to enclave's own in-memory cache called a memtable (Section \ref{sec:kvs}). \algname enables fast KVS read queries because of its shared memory abstraction, so all \texttt{get} operations can directly read from the enclave's memtable without querying other nodes. 




% DataCapsule is a blockchain maintained by multiple secure enclaves, featuring various system optimizations to make communication fast and secure. 
%DataCapsule protects data and communication security by a hash-chained data structure with confidentiality, integrity and provenance guarantee (Section \ref{sec:dc}).  

% Figure \ref{fig:overview} provides an overview of \algname architecture. Distributed worker enclaves are connected by multicast tree(Section \ref{sec:mcast}) For every worker, there are five major components: function executors(Section \ref{sec:faas}), memtable(Section \ref{sec:kvs}), DataCapsule Common Application API(CAAPI) (Section \ref{sec:dc}), circular buffer(Section \ref{sec:circular}), crypto actors(Section \ref{sec:actor}). 
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/Overview.pdf}
    \caption{An overview of \algname's architecture. PSL hosts distributed application workers in different geographic locations. These in-enclave workers communicate with each other by interacting with PSL using \texttt{Put} and \texttt{Get} operations. The KVS updates are propagated by \algname with a secure data structure called DataCapsule. }
    \label{fig:overview}
\end{figure}

% User requests (in C++ or Javascript) are attested and executed by the function executors. The C++ program are directly compiled by linking \algname, and \algname takes an input of plaintext Javascript files and run  in its in-enclave Javascript engine. The input scripts can issue \texttt{put} and \texttt{get}. The \texttt{put} and \texttt{get} interacts directly with an in-memory local cache called memtable. In order for the local changes to memtable to be reflected to the memtables of other authorized enclaves securely, the \texttt{ put}s are handled with DataCapsule CAAPI, a proxy that translates KVS operations to DataCapsule transactions. To increase the throughput, CAAPI dispatches data capsules to the crypto actors. The crypto actors perform computationally heavy cryptographic operations, such as encryption, signing and hashing in parallel. Then they put the processed data capsule into an extremely fast circular buffer to cross the Application-Enclave boundary. The circular buffer propagates the message to all other enclaves by network multicast. 

% Upon receiving a DataCapsule transaction from another enclave, the network client in the untrusted operating system passes the message to the circular buffer. The circular buffer brings the message across the Application-Enclave boundary. The CAAPI verifies the transaction's signature and hash and then updates the memtable with the decrypted message. Since all the updates from other clients are promptly updated to the memtable, the client process can \texttt{get} the latest value among all the enclaves by directly querying the memtable. The consistency is discussed in Section \ref{sec:consistency}.

\subsection{DataCapsule}
\label{sec:dc}

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{figures/DataCapsule_Illustration.pdf}
    \caption{Visual representation of a DataCapsule. Every transaction is encrypted and signed. Every transaction is appended to DataCaspule by including the hash of the previous message as hash pointer.}
    \label{fig:dc_struct}
\end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/DataCapsule_Header.pdf}
%     \caption{Data Structure of a single Data Capsule transaction. Key and Value pair is serialized and encrypted as payload. The senderID, timestamp and payload are hashed by SHA265 Hash. The hash of this message and the previous message by the same sender are signed by ECDSA signature. All the fields collectively constitute a DataCapsule transaction.   }
%     \label{fig:dc_crypto}
% \end{figure}


% \begin{figure}[!tbp]
%   \centering
%   \subfloat[Visual representation of a DataCapsule.]{\includegraphics[width=0.2\textwidth]{figures/DataCapsule_Illustration.pdf}\label{fig:dc_struct}}
%   \hfill
%   \subfloat[Data Structure of a single Data Capsule record.]{\includegraphics[width=0.28\textwidth]{figures/DataCapsule_Header.pdf}\label{fig:dc_crypto}}
%   \caption{ (a) Every record of a DataCaspule is encrypted, signed, appended to the DataCaspule by including the hash of the previous message as a hash pointer. (b) A key-value pair is serialized and encrypted as a payload. The senderID, timestamp and payload are hashed using SHA265. The hash of this message and the previous message by the same sender are signed by ECDSA signature. All the fields collectively constitute a DataCapsule transaction.   }
% \end{figure}



% We propose to use DataCapsule(DC) as the unified standard for inter-enclave communication, due to its confidentiality, integrity, provenance and eventual consistency guarantees. 
A DataCapsule is a secure, append-only blockchain data structure that provides confidentiality, integrity, and provenance inspired by Bitcoin\cite{nakamoto2019bitcoin} and the Global Data Plane\cite{mor2019global}. Figure \ref{fig:dc_struct} shows a visual representation of a DataCapsule hash chain. It contains an append-only hash chain of opaque records, where every record is encrypted and signed. For each record, it has a hash pointer pointing to the previous record of the chain. A single data capsule record is in Figure \ref{fig:dc_crypto}. We assume every DataCapsule writer possesses a private signing key, and all public verifying keys for every other enclave. In addition, all writers share the same symmetric key for both encryption and decryption. The key distribution protocol and bootstrap of in-enclave writers are achieved by enclave attestation (see Section \ref{sec:attestation}). We show that this data structure has the following security properties:
\begin{itemize}
    \item \textbf{Confidentiality} \algname encrypts the serialized key-value pair using the AES encryption scheme. This ensures confidentiality since only other attested trusted execution environments (e.g. attested enclaves) possesses the AES key needed to decrypt the payload.  
    \item \textbf{Integrity} Individual transactions are signed with the ECDSA signing key unique for each individual enclaves (Figure \ref{fig:dc_crypto}). When a transaction is received, other enclaves can verify, using a previously distributed verifying key, that this transaction is produced by a specific enclave. This provides integrity as only the producer enclave can alter the information. 
    \item \textbf{Provenance} Provenance is also ensured as entities can verify which enclave has generated this transaction. 
\end{itemize}


DataCapsules can be easily verified by a third-party without leaking any information about the payload. The third-party verifier can use the \texttt{prevHash} field to trace the entire DataCapsule chain and verify the corresponding hashes and signatures. The DataCapsule data structure can be safely transmitted or stored in an untrusted environment, due to its confidentiality and integrity guarantees. 

\paragraph{CRDT Property of DataCapsule}
The Conflict-Free Replicated Data Type (CRDT) property states that replicas of the database can be merged concurrently without any explicit coordination between replicas, where the replicas can be merged by a function which must be commutative, associative, and idempotent. Due to the append-only design of DataCapsules and the fact that every appended record contains a hash pointer to the previous message, we can define the merge operation to be for each record appended, the merge function uses \texttt{PrevHash} to locate the previous message and append the current message to that previous message. To totally order the appends for messages sharing the same \texttt{PrevHash}, merge primarily sorts by \texttt{Timestamp} and uses \texttt{SenderID} to break ties. The merge function of DataCapsule can be trivially proved to be commutative, associative, and idempotent using induction. An illustration of the merge function is shown in Figure \todonew{TODO figure merge here}.  

The CRDT property of DataCapsule guarantees strong eventual consistency, such that without message loss, two secure enclaves eventually yield an identical copy of the DataCapsule hash chain.


\subsection{Memtable KVS}
\label{sec:kvs}
The Memtable KVS is an in-enclave hash table that \algname aims to replicate consistently with other secure enclaves. The local changes to the memtable are propagated to the memtables of other enclaves and the updates received from other enclaves are reflected to the local memtable. The key-value pairs are stored in plaintext, as the confidentiality and integrity of the memtable are protected by the secure enclave's EPC. 

\paragraph{Memtable as interface to in-enclave applications} In-enclave distributed applications communicate with other enclaves by interacting with the memtable by standard KVS interface: \texttt{put(key,value)} to store a key-value pair and \texttt{get(key)} to retrieve the stored value for a given key. 
\algname assumes the memtable fits in main memory, as its major goal is to relay multiple secure enclaves for communication, instead of durability. 

\paragraph{How memtable works with DataCapsule}
A memtable is an in-memory projection of all the key value pairs in a DataCapsule: if two secure enclaves have identical DataCapsule hash chains, then they have identical memtables. The replication of a Memtable KVS is equivalent to the consistency property of a DataCapsule hash chain.  

As a result, \algname propagates memtable updates to other enclaves securely and consistently by compacting updates into DataCapsule records. \algname uses a notion of DataCapsule Common Application API (CAAPI) as an in-enclave proxy that translates KVS updates to DataCapsule records. For each \texttt{put(key,value)} update to a memtable, the CAAPI compacts the key-value pair into a string and uses AES-encryption to encrypt the string as the DataCapsule payload. The CAAPI completes the rest of the DataCapsule record fields shown in Figure \ref{fig:dc_crypto}, such as hashes and signatures. After completion, the appended DataCapsule record is multicasted to all other secure enclaves. When receiving an update from other enclaves, the CAAPI performs the verification of the DataCapsule hash chain data structure and signatures. If verification succeeds, the decrypted key-value pair is inserted into the memtable. 

% Another view of memtable is a cache of Key-Value pairs in all the DataCapsule records. 
% Directly querying DataCapsule hash chain is computationally heavy pairs, as one needs to trace the DataCapsule hash chain, verify the cryptographic signatures and decrypt the value. Memtable directly stores the plaintext key and value pairs. 

\paragraph{Ordering DataCapsule updates in Memtable} 
%\algname supports multiple ways of assigning a monotonically increasing sequence number to all the transactions, which helps enclaves to reach a consistent view of the order without explicitly exchanging the timestamp information. (1) Timestamp from untrusted operating system by \textit{ocall}s. The overhead for this option is large as mentioned in \ref{sec:background_comm} (2) Timestamp from RDTSC and RDTSCP instructions. These instruction help getting timestamp securely from SGX hardware, but only SGX2 supports these instructions. (3) Lamport Clock. 
As a DataCaspule is an append-only data structure that optimistically collects every update and uses the CRDT property to merge them, \algname needs to order the DataCapsule updates in memtable, and reject the updates that are causally earlier than the ones already in the memtable.  
Naive approaches may lead to undesirable outcomes: for example, replacing the memtable's value whenever a new record arrives leaves the memtable in inconsistent state; ordering two updates by comparing the relative location in the DataCaspule hash chain results in prohibitive overhead. 

To decide the order of the transactions, \algname uses a Lamport logical clock as the default way of timestamping the updates. Without relying on the actual clock \textit{time}, \algname increments a local Sequence Number(SN) whenever there is an update to the local memtable. When receiving a new DataCapsule record, it also synchronizes the SN with the received SN in the record by $SN \gets max(local SN, received SN)+1$. 

Although a vector clock is usually deemed as an upgrade to Lamport logical clocks by including a vector of all  collected timestamps, \algname uses a Lamport clock because a DataCapsule already carries equivalent versioning and causality information, and a vector clock introduces additional complexity and messaging overhead to the system. The reason for not using the actual timestamp from the operating system is that the enclave needs to get a timestamp via ocalls, which costs more than 8,000 CPU cycles due to enclave design \cite{weisse2017regaining}. The RDTSC and RDTSCP instructions from SGX2 are hardware specific, contrary to \algname's goal that supports a variety of TEE hardware. Getting the trusted hardware counter is also expensive, and takes $60-250$ ms \cite{bailleu2019speicher}. 




% \textbf{Epoch-based Freshness} Freshness is a property that protects the database against attackers replaying an old message. Benefited by the SYNC report and hash-chained data structure, \algname guarantees the freshness of the DataCaspule transactions at the level of synchronization epoch. For every DataCapsule message, it contains the hash of the most recent SYNC report or the previous message from the same writer(which eventually points the most recent report along the DataCapsule hash chain). Other enclaves are able to identify if a message is not based on the same SYNC report, and thus verify the freshness of the message. 

%However, a ranged search for multiple matching keys is difficult. % An alternative is tree-based indexing structure, which can provide efficient ranged retrievals, while maintaining and searching tree indices incur higher complexities and overheads.

% Because it uses in-enclave memory for storing, retrieving, and managing key-value pairs, the security 

%Durability is achieved through logging operations to persistent storage. 
%  \texttt{put} and \texttt{get} are handled differently. \texttt{put} operations update local memtable first, and then multicast to and update all remote memtables. On the other hand, \texttt{get} operations only fetch from local memtable.


% To Hanming: what does this paragraph mean?
% \todo{also, don't use sgx in description, asylo supports other enclaves} 
% \textbf{Server-side Encryption} \algname employs a server-side encryption scheme with secure enclaves. Compared to client-side encryption, where the server simply passively stores encrypted data sent by the clients, server-side encryption with SGX provides several benefits. First, server-side encryption provides richer semantics beyond basic operations because the server is able to operate on the stored data. Second, client-side encryption limits usage by a single client. If multiple clients want to decrypt the same data, then a coordination scheme is required among clients to share decrypt key and security metadata. Also, a client is able to remote attest storage server and verify SGX support, the code, and memory state. Thus, the client can be certain that its user data is properly protected within SGX.
    
\subsection{Epoch-based Resynchronization}
\label{sec:consistency}

The CRDT property of a DataCapsule gives a well-defined ordering of all the records in its hash chain. However, even under reliable transmission with appropriate congestion control, the latency of record propagation is not bounded, especially given the wide-area network setting of PSL. This problem is worsened by multiple concurrent writers. For example, many concurrent writers may use the same message as the previous message pointer, and the branching of the hash chain increases the complexity of ordering and verification.  

To reduce the complexity of the DataCapsule hash chain being updated by multiple concurrent writers, \algname branches the DataCapsule data structure by letting every enclave write to its own hash chain. Every append includes a hash pointer to the previous write from the same writer, instead of the previous write from all enclaves. To merge the hash chains maintained by each writer, \algname uses a synchronization (SYNC) report as a rendezvous point. As a result, the resultant DataCapsule hash chain is structured in diamond shape like Figure \todonew{todo, figure here}.  All writers' first writes include a hash pointer to the previous SYNC report, and the next SYNC report includes a hash pointer to the last message of every writer. The SYNC report is useful in the following ways: 
\begin{itemize}
    \item \textbf{Detecting message loss and inconsistency} After an enclave receives a SYNC report, it can use the hash pointers to backtrack to previous messages from the same writer until it reaches the last SYNC report. It detects a message is lost if a hash pointer cannot be recognized during the backtrack. 
    \item \textbf{Detecting freshness of a message} Every message includes a monotonically increasing SYNC report sequence number, which is incremented when a new SYNC report is generated. As a result, one can easily detect the staleness of a message, making \algname aware of a message replay attack. 
\end{itemize}

The usage of SYNC reports establishes a notion of epoch-based resynchronization, a tradeoff between synchronization overhead and consistency. In this consistency model, the user defines a synchronization time interval called an epoch. Between the epochs, the enclaves use the CRDT property of DataCapsules to maintain strong eventual consistency. At the end of an epoch, enclaves cross-validate their own DataCapsule replica with the SYNC report generated by a special Coordinator Enclave (CE). \algname uses the following protocol for SYNC report generation and verification:
\begin{enumerate}
    \item Between epochs, in-enclave writers append to their own hash chain. 
    \item A (CE) keeps a timer for epochs. At the end of the epoch, CE broadcasts a Request To Send (RTS) message to all writer enclaves. 
    \item Every enclave responds to the RTS with an End-of-Epoch (EoE) message, which includes the hash and timestamp of the last message sent by the writer enclave. If there is no update for an enclave within a given epoch, the writer enclave replies with the signature and timestamp of the previous SYNC report.  
    \item After collecting EoE messages from all enclaves, the CE generates a SYNC report that consists of (senderID, last\_message, timestamp) %$(senderID,\ last\_message\_hash,\ timestamp)$ 
    tuples for every writer enclave. The report is hashed and signed by the CE. 
    \item Upon receiving the SYNC report, every writer enclave cross-validates the report with the DataCapsule hash chain and performs loss recovery. Enclaves may query a known enclave or send a broadcast query on the multicast tree.
    \item If the in-enclave writer finishes verifying the SYNC report, it appends the next record with a hash pointer to the previous SYNC report. 
\end{enumerate}
The control messages (RTS, EOE and SYNC reports) are sent, received, and handled by a separate queue with higher priority from other messages. This makes sure that all the enclaves can respond to them promptly (See Section \ref{sec:actor}). 



% \algname guarantees eventual consistency, a relaxed consistency model that if there were no further updates to a specific key $k$, the \texttt{get}$(k)$ from all the in-enclave memtables should return the latest value. Specifically, \algname guarantees eventual last-writer-wins, and the local clients can read the latest received value in the meantime. There are two challenges for \algname to reach eventual consistency: (1) multiple in-enclave writers write to the same DataCapsule hash chain, maintaining consistency requires maintaining consistency of the hash chain  (2) unlike existing database systems, one cannot get timestamps from the untrusted operating system, which is computationally expensive and unsecure. 

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/consistency.png}
%     \caption{An illustration of a scenario in which three enclaves sync when writing to the same DataCapsule. \algname maintains the consistency by End-of-Epoch(EOE) and SYNC messages \todoinline{Replace the figure}}
% %     \label{fig:consistency}
% % \end{figure}

% \textbf{Multiple Writer Consistency}

% To detect loss and inconsistency, \algname periodically performs a synchronization after a certain period of time, or \texttt{epoch}. The synchronization joins the branched DataCaspule chains and allows all worker enclaves to start from the same message for the next epoch. The synchronization is initiated by a Coordinator Enclave(CE). CE is a special worker enclave that is collocated with the multicast router or other worker enclaves. At the end of every epoch, CE broadcasts a Request To Send(RTS) message. Every enclave responds RTS with an End-of-Epoch(EoE) message, which includes the signature and timestamp of the last message sent by the enclave. If there is no update for an enclave within a given epoch, the worker enclave replies with the signature and timestamp of the previous SYNC report. After collecting EoE messages from all enclaves, it generates a SYNC report that consists of $<senderID, last\_signature, timestamp>$ tuples from every worker enclave. Upon receiving the SYNC report, each worker enclave cross-validates the report with its local memtable, and performs loss recovery if (\textit{the signature for a sender does not match} AND \textit{the timestamp on SYNC report is later than the timestamp in its local membtable})

% We note that the existing design can be easily extended to stronger consistency level by blocking on every update, similar to two-phase commit. However, we relax the consistency guarantee for higher throughput as a tradeoff. 



% \subsection{Durability}
% \label{sec:persistence}

% \algname guarantees durability at the granularity of sync epochs: the crashed worker enclave needs to receive the SYNC report from the consistency coordinator, and builds the DataCapsule data structure by querying durability component with the hashes on the SYNC report. The durability component is on the same multicast tree as the worker enclaves. When a worker enclave publishes a DataCapsule update to other enclaves, the durability component records the message and sends an off-tree acknowledgment back to the worker enclave. We propose two durability component designs for \algname, considering the tradeoff of the completeness of the recovered DataCapsule data structure and the overall performance: 

% \paragraph{Non-enclave baseline} The baseline durability component uses a commercial database as the backend, such as Redis or MySQL. When receiving a DataCapsule update from a worker enclave, it verifies the hashes and signatures of the update, and  stores the mapping between the hash of the message and the original message.

% When a worker enclave recovers from a crash, it queries the database with the hashes on the SYNC report, the database returns the corresponding messages. The worker then keep querying the messages using the \texttt{prevHash} field of the received messages from the database. The recovery process is finished until the crashed worker traces to the first message. 

% The security of this design is benefited by the DataCapsule data structure, which an untrusted third-party can easily verify the validity of DataCapsule data structure, and the storing DataCapsule does not compromise the confidentiality and integrity of the actual payload. However, if some key is updated only at the beginning of the DataCapsule chain, the worker needs all messages to recover the entire database. 


% % define level, block, data block, index file, compaction, index, range, hash, DataCapsule, SST files(with its counterpart in our design) 
% % name this component 


% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/Durablity.pdf}
%     \caption{An illustration of the DataCaspule data structure with DCDB. At each SYNC, the memtable is flushed to Level 0 block. The blocks are signed and include a hash pointer to the upper level or the SYNC report. Index files map keys to level blocks and are differentiated by full index and partial index. }
%     \label{fig:persistence}
% \end{figure}

% \paragraph{DataCapsule DB (DCDB)}

% % LSM database archival 
% \algname's \dbname is an in-enclave Log-Structured Merge-Tree(LSM)-based key-value store built on top of the non-enclave baseline, as a separate module on the multicast tree.  
% % Its design is inspired by RocksDB and LevelDB\cite{rocksdb}. 
% LSM is widely used by key-value stores, such as RocksDB\cite{rocksdb}, LevelDB\cite{leveldb} and Speicher\cite{bailleu2019speicher} to secure data storage and query operations.  LSM organizes data into multiple levels, where lower numbered levels are smaller.  New values are added to level-0 (L0) until L0 overflows, at which point some data is merged and sorted into level-1 (L1).  The process repeats for additional levels, though different systems interpret the levels and movement of data in different ways.  In our architecture, levels refer to sorted runs of key-value pairs, where the higher numbered levels are larger and contain older values.  The exception is L0, which is not sorted and has a slightly different structure due to its traditionally small size.  The LSM enables \dbname to naturally move older, staler data further down the tree to larger levels over time.  

% \algname implements \dbname as a special enclave worker that stores and secures the messages from other worker enclaves, in addition to responding to queries from crashed workers. When a new message is published by a worker enclave on the multicast tree, \dbname verifies the message and stores the decrypted key-value pairs in its own memtable. Once the memtable fills, it marks the entire memtable as read-only and serializes the memtable to L0 on disk.  Once L0 is filled, \dbname starts the compaction process.  During compaction, L0 is merged with L1 and the resulting set of keys is sorted.  This sorted set of keys is divided into a number of data blocks, each representing a range of keys.  If L1 overflows as a result of this process, compaction is repeated between L1 and level-2, and so on.  All data blocks are encrypted and stored in the same DataCapsule format used for worker writes, with an index file that maps key ranges to the aforementioned data blocks.  The index is encrypted, signed, and appended whenever an on-disk DataCapsule transaction is written. 

% Beyond RocksDB and Speicher, \dbname also tackles two additional challenges specific to storing data blocks in DataCapsule format: 

% First, since each level is stored as the DataCapsule transaction, \dbname needs the index file to map keys ranges to hashes of DataCapsule transactions, instead of on-disk data blocks (such as SST files in RocksDB and Speicher).  To reduce the overhead for large data sets, \dbname avoids unnecessary rewriting of unchanged data by only appending new or updated key ranges.  \dbname leverages the concept of partial and full indices, with an analogy of shadow paging. Partial indices contain hash pointers only to level blocks that were updated since the last index.  Ranges and levels outside those recently written would map to a hash pointer for the previous index.  Periodically, partial indices are replaced by full indices, which map all ranges and levels to their most up to date respective blocks via hash pointers, irregardless of location within the DataCapsule hash chain. Thus, these full indices act as a checkpoint, guaranteeing that at-worst a read only has to return to the most-recent full index.  \dbname signs all indices when adding them as a new transaction to the DataCapsule.  This creates the additional property that an integrity check only ever needs to verify a single signature.  Since the hashes of transactions are stored in the index, verifying the signature over the index ensures the hashes of the transactions are also correct.  Thus, computing the hash of a transaction and comparing it to the hash stored in the verified index provides a quick way to determine whether a bad actor has tampered with the database.  

% %Second, \dbname needs to () the consistency guarantee by deciding when and how memtable data is converted into DataCapsule transactions.  
% Second, \dbname needs to maintain a consistency view of DataCapsule hash chain when converting memtable into DataCapsule transactions.  
% \dbname tackles this problem by leveraging the consistency mechanism's SYNC report to generate a consistent view of the memtables across all the enclaves.  At periodic SYNCs, \dbname verifies its memtable contains the most up to date key-value pairs based on enclave memtables.  Then, \dbname marks its current memtable as immutable and writes it out to L0.  During this process, enclave progress is halted to ensure the database is consistent with the workers.  After compression and level movements, it appends any newly created blocks as DataCapsule transactions, timestamps each block similar to a standard write from a worker, and generates either a full or partial index.  This index is then written to the DataCapsule, marking the end of \dbname's work at this SYNC.  
% %Before the SYNC ends, the worker enclaves and \dbname are guaranteed to have a consistent view of the data.  If the system needs to restore after a failure, \dbname can trace back through the indices as described below to find the most up to date SST files and rebuild the database. (these are mentioned before, remove them to reduce repetition) 
% The resulting structure is shown by the green blocks in Figure \ref{fig:persistence}.

% To read a value that is not present in a worker's memtable, a \algname worker node sends a request directly to \dbname.  \dbname first pulls the most recent index from the DataCapsule.  If it is a full index, then it verifies the signature over the index and hash of the transaction containing the requested key, then jumps to that block to return the relevant value.  The process for a partial index is similar, except that jumps to prior indices may be necessary if the most recent index does not point to a data block that contains the requested key.  If this occurs, then \dbname verifies the hash of the previous index and repeats this process, though it no longer needs to verify signatures.  
% %If it is a partial index, the process begins similarly by verifying the signature over the index.  \dbname then checks the relevant entry for the requested key and verifies the hash of that transaction.  If present, then the value is returned.  Otherwise, the system traverses back to the next index (partial or full), and repeats this process.  
% This guarantees the integrity of returned values and that the returned value is the most up to date relative to the most recent SYNC. When returning the value, \dbname writes it directly to the requesting worker enclave using the timestamp of the transaction the value was found in, ensuring the correct order of writes and the consistency of the requesting worker's memtable. %When returning the value, \dbname writes it onto the multicast tree using the timestamp of the transaction the value was found in.  This way, newer writes will always take precedence over the returned value, ensuring the correct order of writes and worker memtable values stay consistent. 

\subsection{Multicast Tree}
\label{sec:mcast}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/Multicast Tree.pdf}
    \caption{An illustration of \algname's multicast tree. }
    \label{fig:mcast}
\end{figure}

We conclude this section by showing an overall structure of the multicast tree. Multicast enables one node on the multicast tree to communicate with a group of nodes by routers. Routers receive the message and re-broadcast the message to multiple nodes or routers using static routing rules. The overall structure forms a network multicast tree. The tree-like multicast structure extends the scalability that allows more than one router to handle the communication. \algname is agnostic to the multicast tree topology, as long as a node on the tree publishes the message and every other node can receive that message.  As a result, we can abstract \algname's multicast tree structure as a plane similar to Figure \ref{fig:mcast}. We note there could be optional components on multicast tree: 

\paragraph{Durability Storage} There can be multiple durability storage components on multicast tree to facilitate persistence of the DataCapsule. The most basic durability component uses a commercial database as the backend, such as Redis or MySQL, but PSL has additional designs inspired by RocksDB\cite{rocksdb} beyond the scope of this paper. 

When receiving a DataCapsule update from a worker enclave, it verifies the hashes and signatures of the update, and  stores the mapping between the hash of the message and the original message. When a worker enclave recovers from a crash, it queries the database with the hashes on the SYNC report and the database returns the corresponding messages. The worker then keeps querying the messages using the \texttt{prevHash} field of the received messages from the database. The recovery process is finished when the crashed worker has traced back to the first message. 

The security of this design benefits from the DataCapsule's structure, where an untrusted third-party can easily verify the validity of the DataCapsule's hash chain without compromising the confidentiality and integrity of the actual payload. However, if some key was updated only at the beginning of the DataCapsule chain, the worker would need every message to recover the entire database. 

\paragraph{Third-party Authenticator}
A Third-party Authenticator is an optional component on the multicast tree that can detect the validity of a DataCapsule hash chain without leaking any information about the payload. The third-party authenticator can use the \texttt{prevHash} field and SYNC report to trace the entire DataCapsule chain and verify the corresponding hashes and signatures.



==> discussion.tex <==


\section{Discussion and Future Works}
% Limitations
In this section, we discuss the current limitations of SCL.  

\paragraph{Improving Memory Efficiency:} Previous works on SGX-based KVS involve minimizing the amount of memory inside an enclave \cite{kim2019shieldstore,10.1145/3361525.3361533}. 
While our work focuses more on inter-enclave communication, efficiently using 
available memory and reducing EPC swaps are necessary to the performance of the in-enclave distributed application. We deem this as future \algname work. We shall use or even co-design \algname with alternative TEE platforms and architectures, such as Keystone \cite{lee2019keystone} or Penglai \cite{fengscalable}, to solve this issue. 

\paragraph{Improving Thread Efficiency:} \algname makes use of multi-threading to improve the overall throughput of the inter-enclave communication. For example, the circular buffer requires two enclave threads and two host threads to pass messages to the enclave, and the performance of \algname depends heavily on the number of crypto actors used in the cryptographic pipeline. When there is no active task for the aforementioned threads, they keep spinning and waste CPU cycles. 
While using many threads in not a problem in the modern cloud environment, considering \algname can be deployed on less powerful machines(such as edge servers), 
improving the thread efficiency becomes a valid research problem. We can use conditional variables and wake up the sleeping thread only if needed to reduce the waste of CPU resources. 



%Our work focused more on the inter-enclave communication and providing consistency between several key-value pairs across enclaves. We use an in-memory KVS inside the enclave, which includes the data structure of the entire hash table. We trade-off the memory limitation of the client with the faster communication (i.e. \textit{put()}/\textit{get()}) to the KVS. 

% \textbf{Memory Overhead}: One other limitation is that we replicate key-values across enclaves. Previous work allowed multiple clients to share the same database \cite{10.1145/3361525.3361533}. Because we place the KVS inside the enclave for faster access, we replicate the KVS across the enclaves (i.e. the same key-value pair is stored across all enclaves). This creates a memory overhead of factor of \texttt{N}, where \texttt{N} is the number of enclaves.  Again, we sacrifice the memory overhead with efficient communication between enclaves. 



% - our database is replicated - a lot of storage overhead.  
% - we put things inside the enclave's memtable, others put them outside - memory limitation \todoinline{alex}

% \textbf{Hash-Based Indexing}: \algname employs hash-based indexing to benefit from its simple and efficient single-key operations, along with straightforward maintenance. However, it does suffer on ranged query operations. The alternative is to adopt a tree-based indexing scheme. Modifying the indexing scheme for ranged operations could be a future work.

% \vspace{-8pt}
% \subsection{Future Works}

% \textbf{Durability}: Currently, we are lacking durability components in our system. In particular, all storages are currently in-memory and persistent storage is not present. Outside the scope of this project, we have designed a persistent storage component named DataCapsule Server, which provides persistent storage and memtable reconstruction when system crash occurs. This is part of our future work. 

% \textbf{Latency Measurements}: We are lacking latency-related measurements in our evaluation. In particular, latency measurements could reveal the tradeoffs of introducing batching into the our system. The main reason is that we are limited by time constraints. Adding latency measurements to our experiments is part of our future work.

% \textbf{Extended Support for Containers and Hardware Backends}: In the future, we wish to create support for SGX-based containers like Scone or Graphene, that can hook into our KVS infrastructure easily \cite{tsai2017graphene} \cite{arnautov2016scone}. Furthermore, we wish to support different hardware backends other than SGX to create TEEs like ARM TrustZone or Keystone. Luckily, Asylo is hardware agnostic, so doing this should require little modification in our existing code base. 

%- Obliviousness (ObladiDB, 
% - Container support + Different hardware backends
\todoinline{alex}
% rocksdb 
% 


==> evaluation_v1.tex <==

\section{Evaluation}
%We evaluate our system with an end-to-end benchmark, circular buffer and crypto actors microbenchmark, and a case study on Fog Robotics Motion Planner. We use specific experiment setup for each experiment.
\algname leverages DataCaspules as the data representation to support inter-enclave communication. To quantify the benefits and limitations, we ask: 
% \begin{itemize}
%     \item 
%     \item 
%     \item  
% \end{itemize}
(1) How does \algname perform as a KVS(\S\ref{sec:e2eb})? 
(2) How do circular buffers (\S \ref{sec:circularb}), crypto actors, and batching (\S \ref{sec:actorb}) affect the overhead?  (3) How much does \algname pay to run in-enclave distributive applications(\S \ref{sec:mplambda})?
\subsection{End-To-End Benchmark}
\label{sec:e2eb}
\paragraph{Experiment Setup:} We evaluate KVS's on Azure DCsv2 instances, equiped with Intel(R) Xeon(R) E-2288G CPU @ 3.70GHz with 4 physical cores (8 logical threads). The processor has 32K instruction and data caches, a 256K L2 cache, a 16MB shared L3 cache, and 32GB memory. The machine uses Ubuntu 18.04.5 LTS 64bit with Linux 5.4.0-1048-azure. We run Asylo version 0.6.2. The evaluation is conducted with the baseline durability component. We report the average of experiments that are conducted 10 times. All throughput numbers are in \textbf{log} scale.

\paragraph{Benchmark Design:} End-to-end evaluation starts when the client issues the first request, and ends when the client receives its last request's response from the server. We evaluate the performance using a workload generated by YCSB workload generators. Due to the difference between \texttt{get} and \texttt{put} operations, we evaluate different Read-Write ratios: 100:0, 95:5, 50:50 , 5:95, and 0:100. All workloads comply zipfian distribution, where keys are accessed at non-uniform frequency.

We compare fully optimized \algname against the following baselines: (1) \textbf{Redis+GrapheneSGX}: we run Redis on Graphene \cite{tsai2017graphene} as the SGX-based container service. we enable the switchless option for crossing Application-Enclave boundary. However, we note that this benchmark has \underline{weaker} security model that the communication is not encrypted, hashed and signed.  (2) \textbf{Non-optimized \algname}: we run \algname without batching or crypto actors. This gives the baseline of \algname without optimization mechanisms. For all three KVS's, we evaluate them based on the total throughput of the KVS consisting of two nodes, each on a separate physical machine. Code is compiled with \texttt{copt=-O3}.

\begin{figure}
\vspace*{-0.5 cm}
    \centering
    \includegraphics[width=0.85\linewidth]{figures/e2e.pdf}
    \caption{A bar chart that shows end-to-end benchmark among 1) Fully optimized SCL, 2) Non-optimized SCL, and 3) Redis+GrapheneSGX. Throughput numbers are in log scale. The fully optimized SCL is outperforming the other two across almost all workloads.}
    \label{fig:e2e}
\end{figure}

\textbf{Overall Performance} As shown in Figure \ref{fig:e2e}, the fully optimized SCL is outperforming both Redis+GrapheneSGX and the non-optimized SCL across almost all workloads. Comparing fully-optimized and non-optimized SCL, we see that optimized batching and crypto actors have significantly improved \texttt{put} throughput, while leaving \texttt{get} throughput unaffected. In particular, we see an improvement of 81x (2,737 to 223,811) for put-only workloads. Similarly, fully-optimized SCL outperforms Redis+GrapheneSGX in almost all workloads. In particular, we see 1.5x throughput (429,778 / 285,475) for 50:50 workload and 4x throughput (1,606,781 / 397,553) for read-only workload. This demonstrates that SCL's design is efficient to run in enclaves even with cryptographic components such as signature and encryption.  

The only workload where fully optimized SCL is slightly underperforming is at the RW ratio of 95:5. The reason is that cryptographic components cannot be effectively amortized by put requests at this RW ratio. Due to crypto components, the cost of a batch is almost the same regardless of put requests inside. When write ratio is very low (e.g. 5\%), a batch may only contain several put requests, making cost per request higher. As a result, the throughput for 95:5 RW ratio is slightly slower than both 50:50 and 100:0.
 
\subsection{Circular Buffer Microbenchmark}
\label{sec:circularb}
\paragraph{Benchmark Design:} The circular buffer provides efficient application-enclave communication. We compare the performance of the circular buffer with the SGX SDK baseline and the state-of-the-art HotCall. We evaluate them based on the number of clock cycles required for communications in both the application to enclave direction and vice versa.

\paragraph{Overall Performance:} As shown in Table \ref{table:microbenchmark}, baseline SGX SDK incurs a significant overhead of over 20,000 clock cycles from application to enclave, and over 8,600 clock cycles from enclave to application. For both directions, HotCall is able to reduce the overhead to under a thousand clock cycles. Our circular buffer reduces overheads even further. Our solution only requires 461.1 and 525.54 clock cycles from application to enclave and vice versa. Compared to state-of-the-art HotCall, our solution provides 103\% and 44\% improvements, respectively.

\begin{table}
  \begin{tabular}{| p{0.15\textwidth} | p{0.13\textwidth} | p{0.13\textwidth} |}
    \hline
     \textbf{\# of clock cycles}  & \textbf{App to Enclave} & \textbf{Enclave to App} \\
    \hline
    \textbf{SGX SDK} & 20515.02 & 8608.57 \\
    \hline
    \textbf{HotCalls} & 936.89 & 757.96 \\
    \hline
    \textbf{Circular Buffer} & 461.10 & 525.54  \\
    \hline
\end{tabular}
\caption{\label{table:microbenchmark} \textbf{Circular Buffer Microbenchmark} We evaluate the number of clock cycles required for communications between the enclave and application in both directions.}
\end{table}

\subsection{Actors and Batching Microbenchmark}
\label{sec:actorb}
\paragraph{Benchmark Design:} To eliminate effects of other factors, we conduct the actor and batching microbenchmark with operations generated within the system, and on one node. We measure the throughput and latency by measuring the time difference between when a operation is generated and before it is multicasted to other nodes. We use SGX mode where a KVS client sends a series of operations. This experiment consists of 0:100 \texttt{put} only operations because \texttt{get} operations only require a simple lookup in the local in-memory memtable, which does not benefit from actors and batching. In more detail, a \texttt{put} operation requires the system to update a local memtable, encrypt, compute a hash, sign, use a circular buffer, and then multicast to other nodes. We use zipfian distributed \texttt{put} operations to evaluate our KVS store. Code is compiled with \texttt{copt=-O2}.

\paragraph{Overall Performance:} As shown in Table \ref{table:batchingbenchmark}, when there is no batching and only one actor is used, the baseline throughput is 919.89 \texttt{put} operations per second, with a latency of 0.282 seconds. As we introduce batching, we are amortizing signing overhead from one signature per \texttt{put} operation to one signature per 10/100/1,000 \texttt{put} operations. As shown in Table \ref{table:batchingbenchmark}, batching dramatically boosts throughput to 12,456.99 ops/s with one actor and batch sizes of 1,000. Meanwhile, we see that four actors with no batching increases throughput from 919.89 ops/s to 2,037.66 ops/s, as well as significantly reducing latency from around 0.282 seconds to around 0.097 seconds. Overall, combining both batching and multiple actors, we can achieve a throughput of 20,220.75 ops/s and a latency of 0.135 seconds.

\begin{table}
  \begin{tabular}{| p{0.15\textwidth} | p{0.08\textwidth} | p{0.08\textwidth} | p{0.08\textwidth} |}
    \hline
     \textbf{Throughput(ops/s)}  & \textbf{1 Actor} & \textbf{2 Actors} & \textbf{4 Actors}\\
    \hline
    \textbf{no batching} & 919.89 & 1,617.94 & 2,037.66 \\
    \hline
    \textbf{batch size of 10} & 6,687.86 & 8,157.17 & 9,440.86 \\
    \hline
    \textbf{batch size of 100} & 11,395.27 & 13,297.86 & 16,509.05 \\
    \hline
    \textbf{batch size of 1000} & 12,456.99 & 18,487.54 & 20,220.75 \\
    \hline
  \end{tabular}
  \newline
  \vspace*{0.2 cm}
  \newline
  \begin{tabular}{| p{0.15\textwidth} | p{0.08\textwidth} | p{0.08\textwidth} | p{0.08\textwidth} |}
    \hline
     \textbf{Latency (s)}  & \textbf{1 Actor} & \textbf{2 Actors} & \textbf{4 Actors}\\
    \hline
    \textbf{no batching} & 0.282 & 0.171 & 0.097 \\
    \hline
    \textbf{batch size of 10} & 0.227 & 0.207 & 0.195 \\
    \hline
    \textbf{batch size of 100} & 0.093 & 0.102 & 0.106 \\
    \hline
    \textbf{batch size of 1000} & 0.262 & 0.172 & 0.135 \\
    \hline
  \end{tabular}
\caption{\label{table:batchingbenchmark} \textbf{Actors and Batching Microbenchmark} We evaluate the throughput (ops/s) and latency (s) of various batching and actors setup.}
\end{table}

\subsection{Case Study: Fog Robotics Motion Planner}
\label{sec:mplambda}
In robotics, motion planning algorithms~\cite{Choset2005_Book} compute collision-free paths for a robot to get from a start to a goal \emph{configuration}, where a configuration refers to the complete specification of the robot's degrees of freedom (e.g. joint angles, position in space).
A highly successful class of motion planners are sampling-based.  These motion planners work by randomly sampling configurations and connecting them into a graph of collision free paths. %\todoinline{This paragraph and figure are directly copied from FogROS paper. Need to paraphrase. } -Fixed -Jeff
% These planners can be %linearly (and sometimes superlinearly)
% scaled with additional computing cores.
% Using \algname, we deploy a multi-core sampling-based motion planner~\cite{Ichnowski2014_TRO,ichnowski2019mpt} to a 96-core computer in the cloud to solve motion planning problems from the Open Motion Planning Library (OMPL)~\cite{OMPL} (see Fig.~\ref{fig:moption_planning_scenarios}). This planner node subscribes to topics for the collision model of the environment and motion plan operations
% (Fig.~\ref{fig:mp_nodes}).  When the planner node receives a message on any of these topics, it computes a motion plan, and then publishes it to a separate topic.

We experiment with a sampling-based motion planner that is parallelized to run on multiple concurrent serverless processes, \texttt{MPLambda}~\cite{ICRAJeffIcknowski2020}, and modifying it to use SCL. 
% Because we used Asylo, getting \texttt{MPLambda} to work with our KVS did not require too many modifications. 
Most of the porting effort done was to integrate \texttt{MPLambda}'s build system into Asylo. The modification is about 100 LoC. Many system calls that \texttt{MPLambda} uses are proxied by Asylo. 

Using MPLambda with SCL, we compute a motion plan running a fetch scenario in which a Fetch mobile manipulator robot~\cite{Fetch} declutters a desk. We measure the the wall-clock time to first solution (TTFS) returned by the planners. We run this test on an Intel(R) i7-9700K CPU with SGX hardware.
Because the planner uses random sampling, we run the same computation multiple times with different seeds and compute the average latency to reach the first solution. 

We run up to 8 planners, running on separate hosts using SCL and compare this to running MPLamda without SCL. We have an average enclave worker startup time of 4.32s.
We observe an average ~23.1541x slowdown of MPLambda-SCL compared to the baseline MPLambda. MPLambda planners use the Rapidly-exploring random tree (RRT*) \cite{karaman2011samplingbased} algorithm, to search for paths by randomly generating samples from a search space, checking whether the sample is feasible to explore, and adding the sample to a constructed tree data structure. The tree data structure may grow large and take up a significant amount of memory. Memory in SGX is a limited resource and increased memory pressure leads to more misses in the EPC and requiring paging in and out of enclaves frequently.We attribute the significant slowdown not to our SCL performance, but due to the memory limitations of SGX. There is work on limiting the memory usage of RRT* by bounding the memory for the tree data structure,  which we can adopt in future work \cite{10.1109/ICMA.2013.6617944}.


% \begin{figure}
%     \centering
%     \includegraphics[height=46pt]{figures/ompl-Apartment.png}\hfill%
%     \includegraphics[height=46pt]{figures/ompl-cubicles.png}\hfill%
%     \includegraphics[height=46pt]{figures/ompl-Home.png}\hfill%
%     \includegraphics[height=46pt]{figures/ompl-Twistycool.png}%
%     \caption{\textbf{Motion Planning Scenarios in Fog Robotics Case Study}. We run OMPL~\cite{OMPL} motion planning problems as benchmarks shown here.  In each scenario, the motion planner computes a path that consists of 3D translations and rotations for a rigid object.  The scenarios, left-to-right are: Apartment, Cubicles, Home, and Twistycool.}
%     \label{fig:moption_planning_scenarios}
% \end{figure}

\begin{table}
\centering
  \begin{tabular}{| p{0.09\textwidth} | p{0.15\textwidth} | p{0.15\textwidth} |}
    \hline
     \textbf{Planners}  & \textbf{TTFS Baseline (s)} &\textbf{TTFS SCL (s)}   \\
    \hline
    \textbf{1} & 29.187 & 537.484 \\
    \hline
    \textbf{2} & 11.113 & 276.801	 \\
    \hline
    \textbf{4} & 5.878 & 153.641  \\
     \hline
    \textbf{8} & 5.484 & 92.467  \\
    \hline
\end{tabular}
\caption{Motion Planning Benchmarks} % TODO: use booktabs for professional looking tables -JI
\vspace*{-0.1in}
\end{table}

% \begin{table}
% \centering
%   \begin{tabular}{| p{0.05\textwidth} | p{0.12\textwidth} | p{0.09\textwidth} |  p{0.05\textwidth}  |  p{0.09\textwidth} |}
%     \hline
%      \textbf{Plan- ners}  & \textbf{Latency First Solution (ms) } & \textbf{Latency Best Path (ms) }   & \textbf{Best Cost} & \textbf{Cost/Time} \\
%     \hline
%     \textbf{1} & \emph{timeout} & \emph{timeout} & \emph{timeout} & \emph{timeout} \\
%     \hline
%     \textbf{2} & \emph{timeout} & \emph{timeout} & \emph{timeout} & \emph{timeout} \\
%     \hline
%     \textbf{4} & 275,455.5 (2.1x) & 294,767.5 (1.5x)	& 77.8 (1.44x) &	0.000264 (0.93x) \\
%     \hline
%      \textbf{8} & 134,814.33 (0.79x)	& 200,446.67 (1.03x)	& 53.0487 (1.5x) &	0.000265 (1.46x) \\
%     \hline
% \end{tabular}
% \caption{Motion Planning using \algname}
% \end{table}





==> fault-tolerance.tex <==
\section{Durability and Fault Tolerance} 
\label{sec:fault}
In this section, we discuss the semantics of \algname when facing multiple types of failures, and how it can be highly available to in-enclave distributed applications.

% \paragraph{Inconsistency by lost messages}

% Due to the weak consistent nature of DataCapsule, it is possible for memtables to be temporarily inconsistent state. 
% % We guarantee the consistency of the memtable at the granularity of epochs. The messages in \algname can be lost or delayed for arbitrarily long time, but the participants of the communication can detect the lost message by backtracking the hash pointers on the SYNC report and recover from the message loss at the end of every epoch. The mechanism of recovering a lost message depends on the implementation of durability storage, but one possible option is that the enclave sends the hash of the message that requires recovery and how many steps needed for the durability storage to trace back the hash pointer. The durability storage uses an off-multicast-tree private channel to send the batched messages to the enclave. The enclave verify the structure or keep tracing back the hash pointers. 

% Between the end-of-epoch synchronizations, \algname guarantees strong eventual consistency with CRDT property of DataCapsule. For latency-sensitive applications with weak consistency requirements, they may read in the inconsistent value for lower latency. The epoch based consistency of \algname guarantees the strong consistency at the end of the epoch, which the applications that need strong consistency can get the consistent value or even implement mutual exclusion semantics. User may also tune the epoch length, which a shorter epoch may lead to stronger consistency but higher messaging overhead.

\paragraph{SCL Durability with DataCapsule}
All secure enclaves in \algname may fail by crashing or losing network connection, which may fall behind or even leave its in-memory states inconsistent. SCL is durable if a such enclave can recover all of the in-memory states(i.e. the memtable) consistently and catch-up with the on-going communication. Due to the equivalence of DataCapsule hash chain and the memtable shown in Section \ref{sec:kvs}, the durability of SCL is achieved by making DataCaspule hash chain persistent. An analogy to SCL's durability is Write-ahead Logging(WAL) in many databases, 
%should we cite, SOR? ARIES? ... okay now I am reviewing my prelim 
which logs an update persistently before committing to the permanent database. In SCL, DataCapsule is the append-only log that records the entire history of the memtable, which a crashed enclave can use to recover. The crashed enclave can merge its local inconsistent DataCaspule hash chain with the persistent DataCapsule received from other components, such as a third-party durability storage or in-enclave LSM tree DB. The CRDT property of DataCapsule guarantees the consistency of the hash chain after the merge.  

While directly saving and replaying all the past messages in the entire DataCaspule hash chain do not compromise the correctness and security, this approach introduces prohibitive overhead for recovery. In PSL, we use an in-enclave LSM tree, inspired by RocksDB\cite{rocksdb} and Speicher\cite{bailleu2019speicher}, which compacts all the key value pairs into immutable level files on persistent storage. The level files start from Level 0, which corresponds to the most recent key value pairs on the memtable, and overflow to the next level if the current level is full. The in-enclave LSM tree database resides on the same multicast tree and sends an off-channel acknowledgement to a writer enclave when it has made a certain update persistent. 
However, different from all the previous LSM tree implementations, \algname stores the generated level files as DataCapsule record format, which can be thought as another branch on the chain similar to Figure \ref{fig:sync}. 
% or we can draw another one 
This guarantees confidentiality, integrity and provenance that is coherent with all the communication. 
The crashed enclave recovers by directly reading the compacted level files and verifying with the same DataCaspule verification semantics. The usage of in-enclave LSM tree also enables the values for inactive keys to be stored out of the enclave. 

% \algname guarantees durability at the granularity of sync epochs: the crashed worker enclave needs to receive the SYNC report from the consistency coordinator, and builds the DataCapsule data structure by querying durability component with the hashes on the SYNC report. The durability component is on the same multicast tree as the worker enclaves. When a worker enclave publishes a DataCapsule update to other enclaves, the durability component records the message and sends an off-tree acknowledgment back to the worker enclave. We propose two durability component designs for \algname, considering the tradeoff of the completeness of the recovered DataCapsule data structure and the overall performance: 

% \paragraph{Non-enclave baseline} The baseline durability component uses a commercial database as the backend, such as Redis or MySQL. When receiving a DataCapsule update from a worker enclave, it verifies the hashes and signatures of the update, and  stores the mapping between the hash of the message and the original message.

% When a worker enclave recovers from a crash, it queries the database with the hashes on the SYNC report, the database returns the corresponding messages. The worker then keep querying the messages using the \texttt{prevHash} field of the received messages from the database. The recovery process is finished until the crashed worker traces to the first message. 




% \paragraph{Worker Enclave Failure} 
% All secure enclaves in \algname may fail by crashing or losing network connection, which may fall behind or even leave its in-memory states inconsistent. \algname uses semantics of SYNC report to perform recovery. Upon receiving a SYNC report, the secure enclave that just regained network condition can examine the consistency of its local DataCapsule hash chain with the hash pointers on the memtable. If the enclave detects any inconsistency, it catches up with current epoch by the synchronization messages exchanged at the end of the epoch and by replaying the history from the persistence storage using aforementioned message loss recovery mechanisms. 

\paragraph{Coordinator Failure}  The failure of the coordinator only influences the resynchronization interval, but does not influence the strong eventual consistency given by the CRDT property of DataCapsule and the logical timestamp of the memtable. However, one can use multiple read-only shadow coordinators to improve the fault tolerance and to prevent singe point of failure. If multiple consistency coordinators are on the same multicast tree, one consistency coordinator can actively send Request To Sync to the multicast tree. Other consistency coordinators remain in shadow mode until the SYNC report is not sent for an extended period of time. 






% Sec 6 Fault tolerance
% We can have our durability section here
% We can have a naive out-of-enclave database that passively stores everything; enclaves are able to build the memtable states directly from the database. We refer readers to discussion for CapsuleDB/sharding
% Probably we can have semantics like checkpointing (whatever happens to LFS)
% Talk about security guarantees for DataCapsule for data-at-rest
% Worker fails
% * Recover by replaying messages in out-of-enclave database
% Coordinator fails
% * “A very long epoch” - the epoch-based consistency and liveness guarantee will be back as soon as coordinator is back online
% * Can have several shadow coordinators that only passively record states and build up its memtable, and when the active coordinator is down, have another back online


% \paragraph{Fault Tolerance by Replication} Due to the distributive nature of \algname's multicast tree, one can launch multiple non-worker enclaves of the same type to improve the fault tolerance of the overall system. For example, multiple durability storage components passively log all the messages published by the worker enclaves. If one of several storage components crashes, the durability of the overall system still persists. The crashed durability component can still use the same mechanism to recover the missed messages. If multiple consistency coordinators present on the same multicast tree, one consistency coordinator can actively send Request To Sync to the multicast tree. Other consistency coordinators remain in shadow mode until the SYNC report is not sent for an extended period of time. 

==> implementation_v1.tex <==
\section{Implementation}
In this section, we report the implementation of SCL KVS, and the current implementation progress of the PSL project. 
\todo{rewrite this section, our code base is more complete now} 

\subsection{SCL Implementation}
The core SCL KVS code consisted of roughly 4,000 lines of code in C++, excluding the attestation, distributive application implementations, and experiment scripts. We implement the KVS directly on top of Asylo instead of on a containerized enclave environment. This yields a much smaller TCB than related works such as Speicher \cite{bailleu2019speicher}.  Asylo is a hardware-agnostic framework for TEEs, supporting Intel SGX(v1 and v2) and ARM TrustZone. It also provided a POSIX compliant library that made it easier to port existing applications into enclaves. We use ZeroMQ to implement network multicast and communications between Worker Enclaves.


\subsection{Current Progress on PSL}

We implement PSL on top of the SCL code base, yielding 18,000 LoC in C++ with third-party library modifications. We use gRPC to create a secure FaaS Leader Enclave, which can generate HD Wallet keypairs and startup enclave workers.  We use DukTape, an embedded JavaScript engine in C++, to sandbox enclave applications, now that enclaves can directly execute JavaScript code. The implementation of a LSM-based database for DataCapsules is still in progress, so we instead use RocksDB as a backend persistence storage for evaluation, which responds with an acknowledgement when a new DataCapsule record is received. 


==> threat_model.tex <==

\section{Threat Model} 
In this section, we discuss the threat model of PSL. We assume the attackers are typical "cloud/edge attackers" who can listen and tamper with any communications or computations. For example, the attack may come from a compromised operating system or malicious staff in which attackers have full control over the system. \algname guarantees the confidentiality, integrity, and provenance of any data in execution and in transit. Our trusted computation base (TCB) has been reduced to the processor chip, \algname code, and sandboxed application code running in an enclave. Our TCB specifically excludes the operating system managed by the cloud provider. Thus, our system is resilient to malicious privileged attacks from a compromised operating system. By reducing the TCB, our system is also resilient to certain physical attacks, such as cold boot attacks which attempt to exploit DRAM data by freezing the memory chip~\cite{10.1145/1506409.1506429}, or bus probing attacks which exploit the memory channel between the memory chip and the processor~\cite{10.5555/3241094.3241139}. 

\algname guards against message replay attacks and detects DDoS attacks at a granularity of a user-defined time interval (epoch). Every participant in \algname can quickly detect whether a certain message belongs to the corresponding epoch, and verify the message with signatures and hashes. 

We recognize that SGX does suffer from side-channel attack vulnerabilities~\cite{10.1145/3052973.3053007, sgxsdk, tsgx}. \algname does not directly protect users from such side-channel vulnerabilities, but there are various techniques~\cite{10.1145/3052973.3053007,216033, tsgx,10.1145/2897845.2897885} proposed to mitigate risk. In this paper, we consider such vulnerabilities orthogonal from our system design goals.

In addition, we do not consider availability attacks. This is because cloud providers share a common goal with users to reach high availability. Otherwise, the cloud provider could simply unplug the servers. 

For PSL, we require enclave attestation to ensure the integrity of code running inside of an enclave, and we assume, after a reasonably long period of time, information inside a worker enclave may be leaked due to malicious attacks or unintentional information leak. We use per-application key rotation to ensure security isolation between applications. 




% PSL adopts the typical "cloud/edge attackers", who can listen and tamper with any communications or computations. For example, the attack may come from a compromised operating system kernel or a malicious staff in which the attacker have full control over the system. \algname guarantees the confidentiality, integrity, and provenance of any data in execution and in transit. 
% The trusted computation base (TCB) of SCL is limited to the processor chip, PSL code, and sandboxed application code running in an enclave, which explicitly excludes the operating system managed by the cloud provider. The design of SCL guards against message replay attacks and detects DDoS attacks at a granularity of a user-defined time interval (epoch). However, PSL does not guarantees side-channel attack, given that  Intel SGX suffers from various side-channel attack vulnerabilities~\cite{10.1145/3052973.3053007, sgxsdk, tsgx}. However, there are various techniques~\cite{10.1145/3052973.3053007,216033, tsgx,10.1145/2897845.2897885} proposed to mitigate risk.

% Our TCB Thus, our system is resilient to malicious privileged attacks from a compromised operating system. By reducing the TCB, our system is also resilient to certain physical attacks, such as cold boot attacks which attempt to exploit DRAM data by freezing the memory chip~\cite{10.1145/1506409.1506429}, or bus probing attacks which exploit the memory channel between the memory chip and the processor~\cite{10.5555/3241094.3241139}. 

% \algname guards against message replay attacks and detects DDoS attacks at a granularity of a user-defined time interval (epoch). Every participant in \algname can quickly detect whether a certain message belongs to the corresponding epoch, and verify the message with signatures and hashes. 

% We recognize that SGX does suffer from side-channel attack vulnerabilities~\cite{10.1145/3052973.3053007, sgxsdk, tsgx}. \algname does not directly protect users from such side-channel vulnerabilities, but there are various techniques~\cite{10.1145/3052973.3053007,216033, tsgx,10.1145/2897845.2897885} proposed to mitigate risk. In this paper, we consider such vulnerabilities orthogonal from our system design goals.

% In addition, we do not consider availability attacks. This is because cloud providers share a common goal with users to reach high availability. Otherwise, the cloud provider could simply unplug the servers. 

% For PSL, we require enclave attestation to ensure the integrity of code running inside of an enclave, and we assume, after a reasonably long period of time, information inside a worker enclave may be leaked due to malicious attacks or unintentional information leak. We use per-application key rotation to ensure security isolation between applications. 
